Geometric Covering using Random Fields

A set of vectors $S \subseteq \mathbb{R}^d$ is $(k_1,\varepsilon)$-clusterable if there are $k_1$ balls of radius $\varepsilon$ that cover $S$. A set of vectors $S \subseteq \mathbb{R}^d$ is $(k_2,\delta)$-far from being clusterable if there are at least $k_2$ vectors in $S$, with all pairwise distances at least $\delta$. We propose a probabilistic algorithm to distinguish between these two cases. Our algorithm reaches a decision by only looking at the extreme values of a scalar valued hash function, defined by a random field, on $S$; hence, it is especially suitable in distributed and online settings. An important feature of our method is that the algorithm is oblivious to the number of vectors: in the online setting, for example, the algorithm stores only a constant number of scalars, which is independent of the stream length. We introduce random field hash functions, which are a key ingredient in our paradigm. Random field hash functions generalize locality-sensitive hashing (LSH). In addition to the LSH requirement that ``nearby vectors are hashed to similar values", our hash function also guarantees that the ``hash values are (nearly) independent random variables for distant vectors". We formulate necessary conditions for the kernels which define the random fields applied to our problem, as well as a measure of kernel optimality, for which we provide a bound. Then, we propose a method to construct kernels which approximate the optimal one.

==> 0.5changes.tex <==
\section*{changes}

\begin{enumerate}
    \item move 3.5 to appendix (or to the end)
    \item mention LSH in intro/previous work with mathematical proof in the appendix
    \item reconsider 3.8
    \item remedy 3.3, so that the sine field comes right after.
\end{enumerate}

\subsection{Structure:}

\begin{enumerate}
    \item problem statement
    \item preliminaries
    \item grf
    \item sine field
    \item add Tex by Danny (proof)
    \item Add that we can prove the results (where we previously wrote we can't).
    \item Move the sin field earlier. 
    \item Emphasis our analysis is worst case (address the reviwer's comments). 
    \item Emphasize the distributed applicatios
    \end{enumerate}





